A review of heterogeneous data mining for brain disorders

With rapid advances in neuroimaging techniques, the research on brain disorder identification has become an emerging area in the data mining community. Brain disorder data poses many unique challenges for data mining research. For example, the raw data generated by neuroimaging experiments is in tensor representations, with typical characteristics of high dimensionality, structural complexity and nonlinear separability. Furthermore, brain connectivity networks can be constructed from the tensor data, embedding subtle interactions between brain regions. Other clinical measures are usually available reflecting the disease status from different perspectives. It is expected that integrating complementary information in the tensor data and the brain network data, and incorporating other clinical parameters will be potentially transformative for investigating disease mechanisms and for informing therapeutic interventions. Many research efforts have been devoted to this area. They have achieved great success in various applications, such as tensor-based modeling, subgraph pattern mining, multi-view feature analysis. In this paper, we review some recent data mining methods that are used for analyzing brain disorders.

==> table_notation.tex <==
% Table:  List of Notations
\begin{table}[!ht]
\centering
\caption{List of symbols}\label{tab_notation}
\begin{tabular}{ll}
\toprule
Symbol & Definition and Description\\
\midrule
$s$ & each lowercase letter represents a scale\\
$\mathbf{v}$ & each boldface lowercase letter represents a vector\\
$\mathbf{M}$ & each boldface capital letter represents a matrix\\
$\mathcal{T}$ & each calligraphic letter represents a tensor, set or space\\
%$N$ & is the order of $\mathcal{A}\in \mathbb{R}^{I_1} \otimes \cdots \otimes \mathbb{R}^{I_N}$\\
$\otimes$ & denotes tensor product\\
%$\mathbf{a}\otimes \mathbf{b} \otimes \mathbf{c}$ & denotes a third-order rank-one tensor\\
%$\times_{n}$ & denotes $n$-mode product\\
$\left\langle . ,. \right\rangle$ & denotes inner product\\
$\left| . \right|$ & denotes absolute value\\
$\left\| . \right\|_{F}$ & denotes (Frobenius) norm of vector, matrix or tensor\\
%$\phi(.)$  &  denotes the feature mapping\\
%$\kappa(.,.)$ & represents a kernel function\\
%$L$ &  is the number of tensor samples\\
\bottomrule
\end{tabular}
\vspace{-10pt}
\end{table}

